Revealing Unobservables by Deep Learning: Generative Element Extraction Networks (GEEN)

Latent variable models are crucial in scientific research, where a key variable, such as effort, ability, and belief, is unobserved in the sample but needs to be identified. This paper proposes a novel method for estimating realizations of a latent variable $X^*$ in a random sample that contains its multiple measurements. With the key assumption that the measurements are independent conditional on $X^*$, we provide sufficient conditions under which realizations of $X^*$ in the sample are locally unique in a class of deviations, which allows us to identify realizations of $X^*$. To the best of our knowledge, this paper is the first to provide such identification in observation. We then use the Kullback-Leibler distance between the two probability densities with and without the conditional independence as the loss function to train a Generative Element Extraction Networks (GEEN) that maps from the observed measurements to realizations of $X^*$ in the sample. The simulation results imply that this proposed estimator works quite well and the estimated values are highly correlated with realizations of $X^*$. Our estimator can be applied to a large class of latent variable models and we expect it will change how people deal with latent variables.

==> revealing unobservables by deep learning for arxiv/SummaryTable.tex <==
{
\begin{threeparttable}
\begin{tabular}{l*{4}{c}}
 \toprule
 Simulation Name &\multicolumn{3}{c}{corr($\vec{X^*}$, $\vec{\hat{X^*}}$)}
 & corr($\vec{X^*}$, $\vec{X^1}$)\\
  & min & median & max  & \\
 \cmidrule{2-4}
 Baseline  & 0.97  & 0.98 & 0.98 & 0.89  \\

Linear Error  & 0.94  & 0.96 & 0.97 & 0.89  \\

Double Error  & 0.88  & 0.89 & 0.91 & 0.70  \\
\bottomrule
\end{tabular}
\end{threeparttable}
}
